Discovering Pattern Structure Using Differentiable Compositing

Patterns, which are collections of elements arranged in regular or near-regular arrangements, are an important graphic art form and widely used due to their elegant simplicity and aesthetic appeal. When a pattern is encoded as a flat image without the underlying structure, manually editing the pattern is tedious and challenging as one has to both preserve the individual element shapes and their original relative arrangements. State-of-the-art deep learning frameworks that operate at the pixel level are unsuitable for manipulating such patterns. Specifically, these methods can easily disturb the shapes of the individual elements or their arrangement, and thus fail to preserve the latent structures of the input patterns. We present a novel differentiable compositing operator using pattern elements and use it to discover structures, in the form of a layered representation of graphical objects, directly from raw pattern images. This operator allows us to adapt current deep learning based image methods to effectively handle patterns. We evaluate our method on a range of patterns and demonstrate superiority in the context of pattern manipulations when compared against state-of-the-art

==> old.tex <==
We propose a \textit{differential compositing function} that takes an element images set $E$ with carnality N and their respective properties set $P$ and returns an Image $\mathcal{I}_c$. Usually an Image $\mathcal{I}_c$ is composited from L different images each with HxWx4 dimensionality representing RGBA channels using the eq \ref{eq:compositing}
\begin{equation}
        \mathcal{I}_c = \mathcal{C}(\mathcal{SW}(E_i, P_i))
    \label{eq:compositing}
\end{equation}
where C denotes the compositing function and SW denotes the sampling and warping function\\
 
 Sampling and warping function SW output one image $L_i$ for each $E_i$ and $P_i$ .Each of these $L_i$ different Images are generated based on the element image and its respective parameters $P_i$. Each set of parameters $P_i$ represent a warping of the individual element. Such a sampling and warping function should be able to sample from element image $E_i$ warp it based on the parameters $P_i$ differentially. We want the function that outputs $L_i$ to be able to propagate gradients over $P_i$. We first introduce the sampling and warping function SW and then present the compositing function C. \\
Images are indexed in a discrete way, let us denote the indices of the image as $k = (x, y)$ where $k \in \mathbb{Z} $. Given an Image $E_i$ and an Warping function $W$, an Image transformed using $W$ as 
\begin{equation}
        {L_i} ( {\tilde k} ) = \sum_{k}E_i(W(k, P_i))*Weight(\tilde k, W(k, P_i))
    \label{eq:warping}
\end{equation}

Note $E_i(W(k, P_i))$ we are copying the closest pixel from the input element, therefore we do not have any gradients wrt $P_i$.  

We parametrize properties of each each element with its location on the canvas $\tau$ where $\tau \in \mathbb{Z}^2 $ , rotation $\theta$ where $\theta \in \mathbb{R}$ and visibility of the element $\nu$ where $\nu \in (0,1)$. First we warp the indices base on the $\tau$ and $\theta$ value. Since the canvas of the pattern is larger than the element itself we should scale the indices base on the relative sizes. Here size s is the relative width of the element to the whole canvas. 

\begin{equation}
\tilde k =
\begin{bmatrix}
    cos(\theta)  &  -sin(\theta)      \\
    sin(\theta)  &  cos(\theta)      
\end{bmatrix}
*
(k - \tau) / s
    \label{eq:parametrization}
\end{equation}

Observe that $\tilde k \in \mathbb{R}$
\begin{equation}
    \begin{gathered}
        W_{bilinear} = \tilde k_i -|\tilde k_i| \\
        {L_i} ( {\tilde k_i} ) = W_{bilinear} * \sum_{k}E_i(|\tilde k_i|)*Kernel \\
        + (1 - W_{bilinear})*\sum_{k}E_i(|\tilde k_i| + 1 )*Kernel
    \end{gathered}
    \label{eq:bilinear}
\end{equation}


Such a sampling approach would only propagate gradients in the neighbourhood based on the kernel of choice. Without the kernel for a large sampling rate i.e the element in the final composite is smaller than the input then the function would have sampling artifacts and bad gradients with just bilinear sampling. In order to avoid sub sampling errors and have accurate gradient to the neighbours we first weight the pixels using a kernel and then sample them bi-linearly. In our experiments we have observed that a Gaussian distribution weighting yields good results.

Pixels in image $L_i$ that are not sampled from element image $E_i$ are made default 1, helps with compositing operation which are explained next.

Once we have $L_i$ images then we need to composite all these individually sampled elements to form a single pattern, we want such a compositing have been able propagate accurate gradients to properties of one element based on the properties of other elements. \\

After sampling the image we multiple them with the visibility term $\nu \in (0,1)$ to change the intensity of the whole element. Visibility term $\nu $ is constrained using a sigmoid.

\begin{equation}
    \begin{gathered}
        L_i = L_i * \nu  \\
    \end{gathered}
\end{equation} 
Now we multiple the are the image Li to form but he pattern as:
\begin{equation}
    \begin{gathered}
        \tilde{\mathcal{I}_c} = \prod_{1}^{N}(L_i)\\
    \end{gathered}
\end{equation} 
Note that since the default value of pixels in $L_i$ that are not sample from $E_i$ is 0, pixel values of sampled regions do not change because of the addition. $\tilde{\mathcal{I}_c}$ looks like a pattern image with black background to change the background of the pattern we use the alpha channel $\alpha$ of the $\tilde{\mathcal{I}_c}$ as

\begin{equation}
    \begin{gathered}
        \mathcal{I}_c =  \tilde{\mathcal{I}_c}-(1-{\alpha}) + (1-{\alpha})*background \\
    \end{gathered}
\end{equation} 
We multiple the of alpha channel with $\tilde{\mathcal{I}_c}$ because the alpha channel is sampled using eq \ref{eq:bilinear} it is not binary, multiplying with a non binary alpha mask would decrease the pixel intensity creating an artifact.
 
\begin{algorithm}[h]
\SetAlgoLined
\KwResult{Point set $P_{o}$  with element parameters}
 $P \gets Uniform\_Sample(N)$\;
 $I' \gets COMPOSITE(P, Element, Background)$\;
 $L_p = LOSS(Exemplar, I')$\;
 \While{Not Converged}{
  $P \gets P - \lambda  \frac{\partial L_p}{\partial P}$ \;
  $I' \gets COMPOSITE(P, Element, Background)$\;
  $L_p = LOSS(Exemplar, I')$\;
  $P \gets P \cup HoleFill(P)$\;
 }
 \caption{PatternExpansion(Element, Background, N, Exemplar)}
\end{algorithm}

